POEM: Reconstructing Hand in a Point Embedded Multi-view Stereo

Enable neural networks to capture 3D geometrical-aware features is essential in multi-view based vision tasks. Previous methods usually encode the 3D information of multi-view stereo into the 2D features. In contrast, we present a novel method, named POEM, that directly operates on the 3D POints Embedded in the Multi-view stereo for reconstructing hand mesh in it. Point is a natural form of 3D information and an ideal medium for fusing features across views, as it has different projections on different views. Our method is thus in light of a simple yet effective idea, that a complex 3D hand mesh can be represented by a set of 3D points that 1) are embedded in the multi-view stereo, 2) carry features from the multi-view images, and 3) encircle the hand. To leverage the power of points, we design two operations: point-based feature fusion and cross-set point attention mechanism. Evaluation on three challenging multi-view datasets shows that POEM outperforms the state-of-the-art in hand mesh reconstruction. Code and models are available for research at https://github.com/lixiny/POEM.

==> chapters/img_framework_2in1.tex <==
\begin{figure*}[t]
    \begin{center}
        \begin{minipage}[htp]{0.3\textwidth}
        \centering
        \vspace{9pt}
            \resizebox{\linewidth}{!}
            {
                \includegraphics[width=1.0\linewidth]{figs/multi_cams_views.pdf}
            }
            \caption{\textbf{Intersection area of \textit{N} cameras' frustum spaces.} The gray dots represent the point cloud \pt aggregated from \textit{N} frustums. The dark area is the point embedded multi-view stereo. }
            \label{fig:multi_cams_views}
        \end{minipage}
        \quad
        \begin{minipage}[ht]{0.66\textwidth}
            \centering
            \resizebox{1.0\linewidth}{!}{
                \includegraphics[width=1.0\linewidth]{figs/framework.pdf}
                }\vspace{-6 pt}
                \caption{\textbf{\method's architecture.} It contains two stages: (a) hand's keypoints prediction conditioning on multi-view images, and (b) hand's vertices prediction conditioning on the aforementioned keypoints and multi-view images features. For the symbols: {$\mathbf{\bar{p}}, \mathbf{f}, \mathbf{q}, \mathbfcal{P}, \mathbfcal{V}$}'s definition, please refer to \cref{sec:feats_to_points_assignment} and \cref{sec:cross_set_point_transformer}. }
                \label{fig:architecture}
            \end{minipage}
       \vspace{-18pt}
    \end{center}
\end{figure*}
